Hysteresis and Stabillity

Hysteresis can be defined from a dynamical systems perspective with respect to equilibrium points. Consequently, hysteresis naturally lends itself as a topic to illustrate and extend concepts in a dynamical systems course. A number of examples exhibiting hysteresis, most motivated by applications, are presented. Although the examples can be used to construct student exercises, specific questions are listed in an appendix. A brief extension on hysteresis in partial differential equations is also included.

==> tmp_Manuscript_ForGina_2022_April30_abstract.tex <==
\begin{abstract}
 Hysteresis can be  defined from a dynamical systems perspective with respect to  equilibrium points. Consequently, hysteresis naturally lends itself as a topic to illustrate  and extend concepts in a dynamical systems course. A number of examples exhibiting hysteresis, most motivated by applications, are presented. An additional section on hysteresis in partial differential equations is included.  Although the examples can be used to construct student exercises,  specific questions are listed in an appendix.
 \end{abstract}

\begin{keywords}
  Hysteresis, Equilibria, Stability, Eigenvalues, Differential Equations, Dynamical systems
\end{keywords}

\begin{AMS}
97M10, 34C55, 35B35
\end{AMS}


==> tmp_Manuscript_ForGina_2022_April30_header.tex <==
\title{Hysteresis and Stabillity \thanks{Submitted to the editors \today
\funding{The financial support  of  NSERC for the research discussed in this article is gratefully acknowledged.}}}

\author{Amenda Chow\thanks{Department of Mathematics and Statistics, York University, Canada (\email{amchow@yorku.ca}).}
\and Kirsten A. Morris\thanks{Department of Applied Mathematics, University of Waterloo, Canada (\email{kmorris@uwaterloo.ca}).}
\and Gina Faraj Rabbah\thanks{Department of Mathematics, University of Toronto, Canada (\email{gnicole98@gmail.com}). \textcolor{red}{Ask about Gina's institution}}}

% Custom SIAM macro to insert headers
%\headers{Guide to Using  SIAM'S \LaTeX\ Style}{Dianne Doe, Paul T. Frank, and Jane E. Smith}

